TAOS-CI: Lightweight & Modular Continuous Integration System for Edge Computing

With the proliferation of IoT and edge devices, we are observing a lot of consumer electronics becoming yet another IoT and edge devices. Unlike traditional smart devices, such as smart phones, consumer electronics, in general, have significant diversities with fewer number of devices per product model. With such high diversities, the proliferation of edge devices requires frequent and seamless updates of consumer electronics, which makes the manufacturers prone to regressions because the manufacturers have less resource per an instance of software release; i.e., they need to repeat releases by the number of product models times the number of updates. Continuous Integration (CI) systems can help prevent regression bugs from actively developing software packages including the frequently updated device software platforms. The proposed CI system provides a portable and modular software platform automatically inspecting potential issues of incoming changes with the enabled modules: code format and style, performance regressions, static checks on the source code, build and packaging tests, and dynamic checks with the built binary before deploying a platform image on the IoT and edge devices. Besides, our proposed approach is lightweight enough to be hosted in normal desktop computers even for dozens of developers. As a result, it can be easily applied to a lot of various source code repositories. Evaluation results demonstrate that the proposed method drastically improves plug-ins execution time and memory consumption, compared with methods in previous studies.

==> subsection/000_020_author_type2.tex <==

\author{
\IEEEauthorblockN{Geunsik Lim}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea\\
geunsik.lim@samsung.com}
\and
\IEEEauthorblockN{MyungJoo Ham}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea \\
myungjoo.ham@samsung.com}
\and
\IEEEauthorblockN{Jijoong Moon}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea \\
jijoong.moon@samsung.com}
\and
\IEEEauthorblockN{Wook Song}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea \\
wook16.song@samsung.com }
\and
\IEEEauthorblockN{Sangjung Woo}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea \\
sangjung.woo@samsung.com}
\and
\IEEEauthorblockN{Sewon Oh}
\IEEEauthorblockA{\textit{Artificial Intelligence Center (AIC)} \\
\textit{Samsung Research}\\
Seoul, South Korea \\
sewon.oh@samsung.com}
}
